WSAM: Visual Explanations from Style Augmentation as Adversarial Attacker and Their Influence in Image Classification

Currently, style augmentation is capturing attention due to convolutional neural networks (CNN) being strongly biased toward recognizing textures rather than shapes. Most existing styling methods either perform a low-fidelity style transfer or a weak style representation in the embedding vector. This paper outlines a style augmentation algorithm using stochastic-based sampling with noise addition to improving randomization on a general linear transformation for style transfer. With our augmentation strategy, all models not only present incredible robustness against image stylizing but also outperform all previous methods and surpass the state-of-the-art performance for the STL-10 dataset. In addition, we present an analysis of the model interpretations under different style variations. At the same time, we compare comprehensive experiments demonstrating the performance when applied to deep neural architectures in training settings.

==> makefile <==
# --------------------------------------------------------------------
# Usage:
#
#	all	 make pdf file
#	pdf	 make pdf file
#	clean	 remove files
#	clobber  remove everything
#	check	 doubled word and latex syntax check
#	wc	 word count
# --------------------------------------------------------------------

NAME := main
BIBFILES := library.bib
TEXFILES := paper.tex

DISTILLER := ps2pdf

# --------------------------------------------------------------------

SHELL := bash
LATEX := pdflatex
BIBTEX := bibtex -min-crossrefs=100 # avoid separating out crossrefs
DETEX := detex -n
LACHECK := lacheck
DW := dw # ftp://ftp.math.utah.edu/pub/misc/dw.tar.gz
RM := rm -f
WC := wc

# --------------------------------------------------------------------

all: $(NAME).pdf 
pdf: $(NAME).pdf
check: dw syn

$(NAME).pdf: $(NAME).tex $(BIBFILES) 
	@echo '-------------------- latex #1 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- bibtex --------------------'
	$(BIBTEX) $(NAME)
	@echo '-------------------- latex #2 --------------------'
	$(LATEX) $(NAME).tex
	@echo '-------------------- latex #3 --------------------'
	$(LATEX) $(NAME).tex

dw:
	@-$(RM) $(NAME).dw
	@echo '-------------------- doubled words --------------------'
	@for f in $(NAME).tex ;\
	do \
		echo ----- $$f ----- ; \
		echo ----- $$f ----- >> $(NAME).dw ; \
		$(DETEX) $$f  | $(DW) >> $(NAME).dw ; \
	done

syn:
	@echo '-------------------- syntax check --------------------'
	@$(LACHECK) $(NAME).tex

wc:
	@$(DETEX) $(NAME).tex | $(WC)

clean:
	$(RM) *.{blg,dvi,dw,ilg,log,o,tmp,lbl,aux,bbl,lbl}
	$(RM) *.{idx,ind,toc,lof,lot,brf,out,fls,fdb_latexmk,synctex.gz}
	$(RM) $(NAME).pdf
	$(RM) Images/*.pdf orcid-eps-converted-to.pdf

clobber: clean
	$(RM) *~ \#* core

